Don't Take This Out of Context! On the Need for Contextual Models and Evaluations for Stylistic Rewriting

Most existing stylistic text rewriting methods and evaluation metrics operate on a sentence level, but ignoring the broader context of the text can lead to preferring generic, ambiguous, and incoherent rewrites. In this paper, we investigate integrating the preceding textual context into both the $\textit{rewriting}$ and $\textit{evaluation}$ stages of stylistic text rewriting, and introduce a new composite contextual evaluation metric $\texttt{CtxSimFit}$ that combines similarity to the original sentence with contextual cohesiveness. We comparatively evaluate non-contextual and contextual rewrites in formality, toxicity, and sentiment transfer tasks. Our experiments show that humans significantly prefer contextual rewrites as more fitting and natural over non-contextual ones, yet existing sentence-level automatic metrics (e.g., ROUGE, SBERT) correlate poorly with human preferences ($\rho$=0--0.3). In contrast, human preferences are much better reflected by both our novel $\texttt{CtxSimFit}$ ($\rho$=0.7--0.9) as well as proposed context-infused versions of common metrics ($\rho$=0.4--0.7). Overall, our findings highlight the importance of integrating context into the generation and especially the evaluation stages of stylistic text rewriting.

==> sections/5-contextual-evaluation.tex <==
\section{Evaluation of Text Style Transfer with Context}
%\maarten{I would defs have a \textbf{Contextual Rewriting} section that describes the method (i.e., how we set up contextual rewriting), a \textbf{Contextual Evaluation} section that describes the evaluation (both automatic and human). and then you can describe the results in its own section?}

Previous research \cite{madaan2020politeness, reif2021recipe, reid2021lewis} has commonly employed automatic metrics to evaluate rewrites along three major dimensions: (1) style transfer accuracy, (2) meaning preservation, and (3) fluency. Nonetheless, the notion of "meaning preservation" remains ambiguous and exhibits a lack of consistency throughout existing studies.  Some research \cite{li2018delete,sudhakar2019transforming,mir2019evaluating, reif2021recipe, madaan2020politeness} utilize metrics such as \texttt{BLEU}, \texttt{ROUGE}, and \texttt{METEOR} that measure \texttt{n}-gram overlaps and lexical similarity as indicators of meaning preservation. While other studies \cite{wang2019harnessing,reid2021lewis, roy2023conversation} adopt metrics like \texttt{SBERT} and \texttt{BERTScore} measuring semantic similarity of embeddings as proxies for meaning preservation. 

Additionally, these studies often report only one or two metrics, which may not fully capture the nuances of meaning preservation. This could be problematic since these metrics are designed for tasks like machine translation and summarization, which may have different goals and characteristics compared to style transfer. As a result, there is a pressing need for context-aware evaluation metrics. 

In this section, we explore a wide range of \maarten{sentence-level?} automatic metrics, explore incorporating context into these metrics, and propose a simple context-aware metric
Additionally, we conduct human evaluations in which annotators rank the rewritten texts, in the presence of the preceding context, based on target style strength, entity/event-level similarity, intended meaning, and overall naturalness.

\subsection{Automatic Evaluation Metrics}
\maarten{Should we rename these to sentence-level automatic metrics?}
Since the datasets under consideration are reference-free, we evaluate generated rewrites against the original sentence on the following dimensions: 

\maarten{For space, we could make this into paragraphs instead of itemized list}
\begin{itemize}
    %\vspace{-0.3cm}
    \itemsep0.3em 
    \item \textbf{Style Strength:} Following previous studies \cite{li2018delete, madaan2020politeness}, we assess the style strength of rewritten text by examining the target style probabilities (\textbf{Style-Strength}) of the style-classifier. \akhila{should we use transfer accuracy instead? percentage of generated rewrites classified to be in the target domain }\maarten{I think it's not going to paint a different picture, and maybe introduce extra hyperparams of where the decision boundary lies (i.e., is toxicity $>$ .5 toxic? or $>$ .75 ?}
    
    \item \textbf{Lexical Similarity:} To evaluate lexical similarity (\textbf{Lexical}), we use word-overlap metrics use \texttt{ROUGE} \cite{lin2004rouge}, \texttt{METEOR} \cite{banerjee2005meteor} and word error rate \texttt{WER} \cite{zechner2000minimizing}. Lower \texttt{WER} indicates a higher degree of lexical similarity, while higher \texttt{ROUGE} and  \texttt{METEOR} scores signify increased lexical similarity.
    
    \item \textbf{Semantic Similarity:} For measuring semantic similarity (\textbf{Semantic}), we use \texttt{BERTScore} \cite{zhang2019bertscore}, \texttt{SBERT} \cite{reimers2019sentence}, \texttt{BLEURT} \cite{sellam2020bleurt}, as done in previous work. We also consider \texttt{Smatch} \cite{cai2013smatch}, which measures the similarity between two Abstract Meaning Representation (AMR) graphs, providing a distinct, structured perspective on semantic relatedness that complements other semantic similarity metrics.

    \item \textbf{Fluency:} To assess fluency (\textbf{Fluency}), we employ a language model such as GPT-2 \cite{radford}, utilizing perplexity \maarten{can we use NLL (i.e., pplx but not exponentiated?) cause it's easier to write} as the metric, in accordance with previous studies \cite{holtzman2018learning, xu2018dp}. \maarten{This is just perplexity of the sentence, right?} \maarten{Maybe add an equation here? Something like $p_\text{GPT-2}(r)$ but in terms of log probs or perplexities.}
    
    %\item \textbf{Custom Metric:} \akhila{current metric is $\alpha * cosine-sim(orig sent, rewrite) + (1- \alpha) * cosine-sim(context, rewrite)$ }
    
\end{itemize}

\subsection{Contextual Automatic Evaluation Metrics}
%\maarten{I'm thinking we could use the intuition behind fluency and kind of motivate the other metrics like that, basically, saying that generally speaking, meaning preservation should be grounded in context as well. There's different ways you can operationalize that (maybe look at dialogue eval literature for inspiration on how to evaluate broader fit into the general context?), including fluency (pplx), but also, topical relevance wrt to context and original sentence, as well as lexical similarity to context + originak sentence.}
%\akhila{working on it}
%\akhila{include that its context+text vs rewrite; also how to motivate?}
Inspired by the integration of reference-free metrics in dialog evaluation \cite{yeh2021comprehensive, zhao2017learning}, which capture the semantics of both dialogue context and generated responses to assess the response within the dialogue history, we investigate the incorporation of context into automatic evaluation metrics.

\maarten{I don't love subsubsections, can we use paragraphs / itemized lists?}\xuhui{changed}
\paragraph{Contextual Lexical and Semantic Similarity}
Considering the one-to-many nature of suitable rewrites for a specific context, we are interested in devising a straightforward method that evaluates rewrites without excessively penalizing deviations from the original sentence, while still accounting for meaning and relevance within the context. To achieve this, we employ the aforementioned metrics with respect to both the original sentence and the context. Essentially, we examine the lexical and semantic similarity of a rewrite in relation to the combination of \{context + the original sentence\}. \maarten{I think we might want to add explicit names to these methods and list them here. E.g., \texttt{sBERT}$_\mathtt{Ctx}$ or \texttt{ROUGE-Ctx}, etc. Cause otherwise the differences between contextual and acontextual eval metrics aren't super clear.}

\paragraph{Contextual Coherence }
%\akhila{can we use fluency? some papers refer to fluency as just ppl without context}
We are also interested in measuring the contextual coherence of a rewrite of the preceding context. Here, similar to \cite{pang2020towards}, we use a large language model like GPT-2 \cite{} to define contextual coherence as the log-likelihood of the rewrite conditional on the context normalized by the rewrite length. 
\akhila{is this below stuff necessary?} \maarten{Not all of it, but we can defs use an equation that expressed that we're conditioning on the context, so something like $\log p_\text{GPT-2}(r|c)$ or something.}
Suppose a context $c$ contains tokens $\{c_t : t = 1, \dots, T_c\}$ and a rewrite $r$ has tokens $\{r_t : t = 1, \dots, T_r\}$. Let $P$ denote probabilities from GPT-2, then contextual coherence via perplexity $ppl$ is 

\begin{equation}
probs(r | c) = \frac{1}{Tr} \log \frac{P(c, r)}{P(c)} 
\end{equation}
\begin{equation}
    = \frac{1}{Tr} \sum_{t} \log P(r_t | r_{<t}, c)
\end{equation}
\begin{equation}
    ppl = 2^{-\sum_{i=1}^{n} probs_i \log_2(probs_i)}
\end{equation}

%\akhila{\cite{pang2020towards} does this differently by using the 5th percentile to deal with unboundedness - need to adopt; additionally they do "Logical Self-Consistency" as  1 minus the contradiction
%score (context, response) - try this instead of our current entailment score}

\paragraph{Custom Metric}
We present \texttt{ctxt-aware-sim}, a straightforward metric that calculates the weighted sum of the cosine similarity between the embeddings of the rewrite and the original sentence, as well as the cosine similarity between the rewrite and the preceding context's embeddings. \akhila{work in progress, need to swap our contextual semantic sim with coherence maybe}
\akhila{need to motivate this metric, change the formatting}

$cas = \alpha * cosine(orig sent, rewrite) + (1- \alpha) * cosine(context, rewrite)$

\subsection{Human Evaluation}\label{ssec:human-eval-setup}
Similar to automated metrics, most prior work \cite{madaan2020politeness, li2018delete} conducts human evaluation studies without providing annotators with the context, potentially leading to discrepancies in their evaluations due to the need to infer meaning. To address this limitation, we implement a head-to-head comparison methodology in our human evaluation studies for each task, incorporating the preceding context.

In our evaluation, participants are presented with pairs of rewritten sentences, the context and the desired target style attribute. 
They are then asked to rank the two rewrites along various dimensions: 1) target \textit{style strength} (which rewrite best achieves the required style, irrespective of meaning changes), 2) \textit{event-level similarity} (which rewrite best preserves the general events, entities, and relations occurring in the original sentence), 3) \textit{intended meaning} (which rewrite has the closest implied overall message to the original sentence), and 4) \textit{naturalness} (which rewrite feels most natural).
\maarten{The next two sentences feel somewhat redundant wrt to the first paragraph above, maybe we can merge the points into the first paragraph above?}
Including the context in the evaluation process ensures that human evaluators have the necessary information to make informed judgments about the overall quality of the rewritten sentences. This context-aware evaluation strategy aims to yield a more reliable and robust understanding of the performance of different rewriting techniques in real-world applications.


==> sections/6-experiments.tex <==
%We conduct few-shot prompting experiments with two LLMs: GPT 3 \akhila{is text-davinci-003 gpt3 or instruct gpt or gpt3.5? }\maarten{it's GPT-3.5 \cite{ouyang2022}, but we should defs say in a footnote that we use \texttt{text-davinci-003}.} \cite{} and GPT NeoX \cite{} (20B parameters). 
%\subsection{Prompt settings}
%- 2 shot for GPT3
%- 10 shot for gpt neoX

\section{Experiments and Results}
\begin{table*}[t]
    \centering
    \small
    \resizebox*{0.9\textwidth}{!}{
    \begin{tabular}{cc|ccc|cccc|c|c}
        \toprule    
        & & \multicolumn{3}{c|}{Lexical} & \multicolumn{4}{c|}{Semantic} & Style & Fluency  \\\midrule
        & Rewrites & ROU & MET & WER & BERT-S & BLEURT & SBERT & Smatch & Tgt.Probs  & ppl \\ \midrule \midrule
        %& Total & 32, 582 \\ \midrule
        \multirow{3}{*}{\rotatebox{90}{GPT-3.5}} & Acontextual  & \textbf{0.28}&\textbf{0.49}&\textbf{0.91}&\textbf{0.94}&\textbf{0.14}&\textbf{0.73}&<amr>&1.16 & <ppl>\\
        & Contextual & 0.19&0.40&2.14&0.92&-0.27&0.62&<amr>&\textbf{1.17}& <ppl>\\
        & Random Context & 0.18&0.35&3.17&0.91&-0.41&0.52&<amr>&-& <ppl>\\ \midrule\midrule
        \multirow{3}{*}{\rotatebox{90}{NeoX}} & Acontextual  & \textbf{0.45}&\textbf{0.63}&\textbf{0.72}&\textbf{0.95}&\textbf{0.18}&\textbf{0.80}&<amr>&0.7& <ppl>\\
        & Contextual& 0.26&0.42&1.88&0.91&-0.45&0.60&<amr> &\textbf{0.83}& <ppl>\\
        & Random Context & 0.21&0.36&1.90&0.91&-0.56&0.60&<amr>&-& <ppl>\\ \midrule
        %& 0.26&0.42&1.88&0.91&-0.45&0.60&<amr>
    \end{tabular}
    }
    \caption{Acontextual automated metrics results on documents (CNN Daily Mail and Blog Authorship Corpus) for formality}
    \label{tab:auto_formal_doc_acon}
    %\vspace{}
\end{table*}


\begin{table*}[t]
    \centering
    \small
    \resizebox*{0.9\textwidth}{!}{
    \begin{tabular}{cc|ccc|cccc|c|c}
        \toprule    
        & & \multicolumn{3}{c|}{Lexical} & \multicolumn{4}{c|}{Semantic} & \multirow{2}{*}{Custom} & \multirow{2}{*}{Coherence}   \\
        & Rewrites & ROU & MET & WER & BERT-S & BLEURT & SBERT & Smatch  &  &  \\ \midrule \midrule
        %& Total & 32, 582 \\ \midrule
        \multirow{3}{*}{\rotatebox{90}{GPT-3.5}} & Acontextual  & 0.15&0.20&0.87&0.89&-0.62&0.50&<amr> & 0.78& 275.57  \\
        & Contextual & \textbf{0.16}&\textbf{0.23}&\textbf{0.89}&\textbf{0.90}&\textbf{-0.47}&\textbf{0.61}&<amr>&\textbf{0.79}&\textbf{122.09}  \\
        & Random Context & 0.10&0.16&1.06&0.87&-0.82&0.38&<amr>&-&-
        \\ \midrule\midrule
        \multirow{3}{*}{\rotatebox{90}{NeoX}} & 
        Acontextual  &0.23&0.24&0.84&0.89&-0.66&0.52&<amr>&0.81&<recom>  \\
        & Contextual &\textbf{0.25}&\textbf{0.28}&\textbf{0.83}&\textbf{0.90}&\textbf{-0.57}&\textbf{0.62}&<amr>&0.81 &<recom>  \\
        & Random Context &0.16&0.19&0.92&0.87&-0.88&0.42&<amr>&-&-\\ \midrule
        
    \end{tabular}
    }
    \caption{Contextual automated metrics results on documents (CNN Daily Mail and Blog Authorship Corpus) for formality}
    \label{tab:auto_formal_doc_con}
    %\vspace{}
\end{table*}




\begin{table*}[t]
    \centering
    \small
    \resizebox*{0.9\textwidth}{!}{
    \begin{tabular}{cc|ccc|cccc|c|c}
        \toprule    
        & & \multicolumn{3}{c|}{Lexical} & \multicolumn{4}{c|}{Semantic} & Style & Fluency  \\\midrule
        & Rewrites & ROU & MET & WER & BERT-S & BLEURT & SBERT & Smatch & Tgt.Probs & ppl \\ \midrule \midrule
        %& Total & 32, 582 \\ \midrule
        \multirow{3}{*}{\rotatebox{90}{GPT-3.5}} & Acontextual  & \textbf{0.22}&0.41&1.23 & 0.91&-0.14&0.72&<amr>& 1.34 & <ppl>  \\
        & Contextual & 0.16&0.38&2.67&0.90&-0.29&0.67&<amr>&1.38 & <ppl> \\
        & Random Context & 0.15&0.32&3.72&0.89&-0.43&0.58&<amr>&-& <ppl>\\ \midrule\midrule
        \multirow{3}{*}{\rotatebox{90}{NeoX}} & Acontextual  & \textbf{0.36}&0.55&0.98&0.92&-0.04&0.78&<amr>&0.73 & <ppl>\\
        & Contextual & 0.24&0.41&1.97&0.90&-0.44&0.65&<amr>&0.90& <ppl> \\
        & Random Context &0.23&0.40&2.70&0.90&-0.49&0.60&<amr>&-& <ppl>\\ \midrule
        
    \end{tabular}
    }
    \caption{Acontextual automated metrics results on Reddit conversations for formality}
    \label{tab:auto_formal_reddit_acon}
    %\vspace{}
\end{table*}

\begin{table*}[t]
    \centering
    \small
    \resizebox*{0.9\textwidth}{!}{
    \begin{tabular}{cc|ccc|cccc|c|c}
        \toprule    
        & & \multicolumn{3}{c|}{Lexical} & \multicolumn{4}{c|}{Semantic} & \multirow{2}{*}{Custom} & \multirow{2}{*}{Coherence}   \\
        & Rewrites & ROU & MET & WER & BERT-S & BLEURT & SBERT & Smatch  &  &  \\ \midrule \midrule
        %& Total & 32, 582 \\ \midrule
        \multirow{3}{*}{\rotatebox{90}{GPT-3.5}} & Acontextual  & 0.14&0.24&0.95&0.88&-0.66&0.56&<amr> & 0.67& 215.57  \\
        & Contextual & 0.14&0.27&0.91&0.89&-0.46&0.66&<amr>&0.71&62.49  \\
        & Random Context & 0.11&0.20&1.58&0.87&-0.77&0.47&<amr>&-&-
        \\ \midrule\midrule
        \multirow{3}{*}{\rotatebox{90}{NeoX}} & Acontextual  &0.22&0.29&0.88&0.88&-0.66&0.58&<amr>&0.72&<recom>  \\
        & Contextual &0.21&0.29&0.88&0.89&-0.60&0.64&<amr>&0.72 &<recom>  \\
        & Random Context & 0.17&0.22&1.29&0.87&-0.86&0.46&<amr>&-&-\\ \midrule
        
    \end{tabular}
    }
    \caption{Contextual automated metrics results on Reddit conversations for formality}
    \label{tab:auto_formal_reddit_con}
    %\vspace{}
\end{table*}
\subsection{Rewriting Setup}
% models, n 
\maarten{should we perhaps move this section to the modeling setup section (\S\ref{sec:modeling-setup})?}
We conduct few-shot prompting experiments with two LLMs: GPT-3.5 \footnote{We use \texttt{text-davinci-003}}\cite{ouyang2022training} \akhila{is this correct?}\maarten{yup I think so!} and GPT NeoX \cite{black2022gpt} (20B parameters). 
For GPT-3.5, we utilize 2 few-shot examples primarily to generate rewrites in the desired format, while for GPT-NeoX, we use 10 few-shot examples. All these few-shot instances are manually constructed. To generate contextual rewrites, the model is prompted with examples containing the preceding context, the original sentence to be rewritten, an instruction specifying the required style, and a sample rewrite. For acontextual rewrites, we omit the preceding context, and for rewrites with a random context, we substitute the actual preceding context with a random one from the dataset. \maarten{note, some of this was already said in \S\ref{sec:modeling-setup}?}

\subsection{Automated Evaluation Results}
\akhila{@Maarten, I need help with this section to highlight our takeaways from the automated metrics. Right now it feels very flat and not punchy enough}
\maarten{so for this section, I recommend starting small and just listing the main trends and results you notice, without much fluff (maybe start with a bulleted list first, then rank the findings in terms of most relevant to our general point of our paper (e.g., contextual metrics prefer contextual rewrites) to least relevant (GPT-3.5 and GPT-Neo don't perform the same).TBH what you have is pretty good already, I think you could just condense things a little more!}
% add results, take aways
We examine automatic evaluation metrics in two stages: first, by conducting a head-to-head comparison between the rewrite and the original sentence, referred to as `Acontextual evaluation'; and second, by comparing the rewrite to the combination of the preceding context and the original sentence, termed as `Contextual evaluation'. This two-stage approach allows for a comprehensive assessment of the rewrites, taking into account both the original sentence and the contextual information.

We observe that acontextual rewrites tend to achieve higher scores compared to contextual rewrites when evaluated using acontextual lexical and semantic similarity-based automated metrics, as shown in Table \ref{tab:auto_formal_doc_acon} (results on document-based context for formality). Conversely, contextual rewrites receive higher or equivalent scores when assessed using contextual lexical and semantic similarity-based automated metrics, as illustrated in Table \ref{tab:auto_formal_doc_con} (results on document-based context for formality). This pattern remains consistent across all datasets and for all three tasks. It is important to note that these lexical and semantic metrics only partially represent meaning preservation. Nonetheless, we have endeavored to encompass a broad range of metrics that measure various aspects of meaning.

\akhila{how to compare gpt-3.5 vs gpt neoX }

We also observe that contextual rewrites exhibit a stronger style strength compared to acontextual rewrites, a trend that is consistent across all datasets. Additionally, contextual rewrites tend to be more coherent with the preceding context and achieve higher scores on our custom \texttt{context-aware-sim} metric.

\maarten{This is wonderful! you could potentially use these two insights, turn them into \textbackslash paragraphs, and move the discussion of specific results under each of these points. See my voice message i sent in slack}
From these observations, we derive two key insights: 1) Commonly used automated metrics are not compositional or contextual; and may not always provide a comprehensive evaluation, necessitating the incorporation of context into the assessment of rewrites  2) There are simple ways to include and design metrics which integrate context into automated metrics. In Section \ref{sec:human_eval}, we show that annotators prefer contextual rewrites over acontextual rewrites, when grounded in context. 
\maarten{Should we say something about the differences between the three tasks? And somethign about the differences between document context and conversational context?}

% which are partially representative of meaning preservation \akhila{need a comment here to say these are not entirely meaning preserving representative but are the closest we can get}
\subsection{Human Evaluation with Context}
\akhila{@Maarten, I need help with this section too..}
\maarten{I think same advice as above, focus on the one or two main takeaways for these results, which you're already doing! We can just condense some of the points!}

\begin{figure}[t]
\centering
\begin{subfigure}{\columnwidth}
\includegraphics[width=\columnwidth,clip]{Figures/formality_barh.pdf} 
\caption{Formality}
\label{fig:human_formality}
% \vspace{1em}
\end{subfigure}

\begin{subfigure}{\columnwidth}
\includegraphics[width=\columnwidth,clip]{Figures/toxicity_barh.pdf}
\caption{Toxicity}

\label{fig:human_toxicity}
\end{subfigure}
\caption{Human Evaluation \akhila{add caption}\maarten{nitpick: the fonts are a little small, and the bars are quite spaced out; we could probably condense things a little more! But these are super pretty already!}}
\vspace{-10pt}
\label{fig:human_eval}
\end{figure}

\maarten{we have to consolidate the info we give here and what we discussed in \S\ref{ssec:human-eval-setup}, to make sure we're not repeating things.}
In order to obtain a direct assessment of style transfer quality in both contextual and acontextual rewrites, we carry out a human evaluation. We present human evaluators with three elements: a preceding context, the original sentence to be rewritten, and the desired target style attribute. They are then asked to rank the two rewrites based on target style strength, event-level similarity, intended meaning and overall naturalness \maarten{as described in \S\ref{ssec:human-eval-setup}}. For each task, we sample approximately 50 examples from each dataset (i.e., each context type). We employ three workers per rewrite pair and use Cohen's kappa to measure inter-annotator agreement \footnote{Interrater agreement was Cohen’s $\kappa$=\akhila{insert} on average} for each head-to-head evaluation.

As shown in Figure \ref{fig:human_eval}, it is evident that annotators generally prefer contextual rewrites over acontextual ones. Moreover, annotators believe that the overall intended meaning, which we argue should be classified as 'meaning preservation,' is best captured through contextual rewrites. Conversely, for event-level meaning concerning entities and events, acontextual rewrites are favored. We hypothesize that when LLMs are not provided with any context, they tend to exhibit greater similarity on an $n$-gram level with the original sentence, which assists in preserving the events. This is also demonstrated by our acontextual automated evaluation.





